Bayes Linear Analysis for Statistical Modelling with Uncertain Inputs

Statistical models typically capture uncertainties in our knowledge of the corresponding real-world processes, however, it is less common for this uncertainty specification to capture uncertainty surrounding the values of the inputs to the model, which are often assumed known. We develop general modelling methodology with uncertain inputs in the context of the Bayes linear paradigm, which involves adjustment of second-order belief specifications over all quantities of interest only, without the requirement for probabilistic specifications. In particular, we propose an extension of commonly-employed second-order modelling assumptions to the case of uncertain inputs, with explicit implementation in the context of regression analysis, stochastic process modelling, and statistical emulation. We apply the methodology to a regression model for extracting aluminium by electrolysis, and emulation of the motivating epidemiological simulator chain to model the impact of an airborne infectious disease.

==> Arxiv version 3 - UI Paper 09.05.23/Definitions.tex <==
%%% List of Definitions %%%

% Begin and end equations, lists, figures etc.
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{eqnarray}}
\newcommand{\ea}{\end{eqnarray}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bn}{\begin{enumerate}}
\newcommand{\en}{\end{enumerate}}
\newcommand{\bfi}{\begin{figure}}
\newcommand{\efi}{\end{figure}}

% Extended subfigure commands.
% subfig - file, prop. column width, scale, vertical space reduction to caption, caption, label, space underneath caption..
\newcommand{\subfig}[6]{\begin{subfigure}{#2\columnwidth}
\centering
\includegraphics[scale=#3]{#1}
\vspace{#4cm}
\caption{\footnotesize{#5}}
\label{#6}
\end{subfigure}}

% File where figures are stored.
\newcommand{\figfile}{R_Code_and_Figures/Figures}

% BL Expectations, variances etc.
\def \expectation  {\textrm{E}} 
\def \variance {\textrm{Var} }
\def \covariance {\textrm{Cov} }
\def \correlation {\textrm{Corr} }
\newcommand{\e}[1]{\ensuremath{{\rm E}[#1]}}
\newcommand{\ed}[2]{\ensuremath{{\rm E}_{#1}[#2]}}
\newcommand{\edhat}[2]{\ensuremath{{\hat{\rm E}}_{#1}[#2]}}
\newcommand{\var}[1]{\ensuremath{{\rm Var}[#1]}}
\newcommand{\vard}[2]{\ensuremath{{\rm Var}_{#1}[#2]}}
\newcommand{\vardhat}[2]{\ensuremath{{\hat{\rm V}\rm{ar}}_{#1}[#2]}}
\newcommand{\corr}[2]{\ensuremath{{\rm Corr}\left[#1,#2\right]}}
\newcommand{\corrd}[3]{\ensuremath{{\rm Corr}_{#1}\left[#2,#3\right]}}
\newcommand{\cov}[2]{\ensuremath{{\rm Cov}[#1,#2]}}
\newcommand{\covd}[3]{\ensuremath{{\rm Cov}_{#1}\left[#2,#3\right]}}
\newcommand{\aed}[2]{\ensuremath{{\rm \hat{E}}_{#1}[#2]}}
\newcommand{\avard}[2]{\ensuremath{{\rm \hat{V}ar}_{#1}[#2]}}

% Specifically with F
\newcommand{\eF}[1]{\ed{\bF}{#1}}
\newcommand{\varF}[1]{\vard{\bF}{#1}}
\newcommand{\covF}[2]{\covd{\bF}{#1}{#2}}
\newcommand{\eFX}[1]{\ed{\bF \cup \bX}{#1}}
\newcommand{\varFX}[1]{\vard{\bF \cup \bX}{#1}}
\newcommand{\covFX}[2]{\covd{\bF \cup \bX}{#1}{#2}}

% Full Bayesian expectations, variances etc.
\def \fbexp { \mathbb{E} }
\def \fbvar { \mathbb{V}ar }
\def \fbcov { \mathbb{C}ov }

% Conventional notations.
\def \indicator { \mathbb{I} }
\def \identity { \boldsymbol{I} }
\def \independent {\perp\!\!\!\perp} 
\def \GP { \mathcal{GP} }
\def \normal { \mathcal{N} }
\def \real { \mathbb{R} }
\def \det {\textrm {det}}
\def \trace {\textrm {trace}}
\def \vect {\textrm {vec}}

% Specific
\def \ind {\indicator}
\def \half {\frac{1}{2}}
\def \mn {\frac{m^2}{n}}
\def \tmn { t_{mn} }
\def \tmx { t_{mx} }
\def \Tmn { T_m }
\def \Tmx { T_{mx} }

% Ensure math mode.
\newcommand{\cm}[1]{\ensuremath{ { #1 }}}

% Greek letters.
\def \al { \alpha }

% Mathcal letters.
\newcommand{\ma}{\mathcal{A}}
\newcommand{\mb}{\mathcal{B}}
\newcommand{\md}{\mathcal{D}}
\newcommand{\mk}{\mathcal{K}}
\newcommand{\mt}{\mathcal{T}}
\newcommand{\mx}{\mathcal{X}}
\newcommand{\my}{\mathcal{Y}}
\newcommand{\mz}{\mathcal{Z}}

% Bold letters.
\def \bbe { \mathbf{b} }
\def \bc { \mathbf{c} }
\def \bd { \mathbf{d} }
\def \bof { \mathbf{f} }
\def \bg { \mathbf{g} }
\def \bh { \mathbf{h} }
\def \bk { \mathbf{k} }
\def \bt { \mathbf{t} }
\def \bu { \mathbf{u} }
\def \bv { \boldsymbol{v} }
\def \bw { \boldsymbol{w} }
\def \bx { \mathbf{x} }
\def \by { \mathbf{y} }
\def \bz { \mathbf{z} }
\def \bA { \mathbf{A} }
\def \bB { \boldsymbol{B} }
\def \bC { \boldsymbol{C} }
\def \bF { \mathbf{F} }
\def \bG { \boldsymbol{G} }
\def \bH { \mathbf{H} }
\def \bK { \mathbf{K} }
\def \bL { \mathbf{L} }
\def \bT { \mathbf{T} }
\def \bU { \mathbf{U} }
\def \bW { \boldsymbol{W} }
\def \bX { \mathbf{X} }
\def \bY { \mathbf{Y} }
\def \bZ { \mathbf{Z} }
\def \bb { \bm{\beta} }
\def \bGa{ \bm{\Gamma} }
\def \bDe { \boldsymbol{\mathit{\Delta}} }
\def \bet { \eta }
\def \beps { \bm{\epsilon} }
\def \br { \bm{\rho} }
\def \Sig { \boldsymbol{\mathit{\Sigma}} }
\def \bth { \bm{\theta} }
\def \bphi { \bm{\phi} }
\def \bxi { \xi }
\def \bTh { \boldsymbol{\mathit{\Theta}} }
\def \bO { \boldsymbol{\mathit{\Omega}} }
\def \bizero { \boldsymbol{\mathit{0}} }
\def \bzero { \mathbf{0} }
\def \mbX { \mathbb{ X } }
\def \mbZ { \mathbb{ Z } }

% Composite and component simulators and inputs/outputs.
\def \com { \bh }  % Composite simulator bold h.
\def \cin { \bz } % Composite simulator input bold z.
\def \cout { \by } % Composite simulator output bold y.
\def \comin { \com(\cin) } % Composite simulator with input.
\def \simr { \bof } % Component simulator bold f.
\def \siin { \bx } % Component simulator generic input bold x.
\def \simrin { \simr(\siin) } % Component simulator with input. 
\def \simri { \simr^i } 
\def \simrj { \simr^j }
\def \simrcin { \simr^1(\bz) } 
\def \bez { \bt^E(\bz) }
\def \bvz { \bt^V(\bz) }
\def \cx { \bc(\bx) }
\def \cxp { \bc(\bx') }
\def \fx { \simr(\bx) }
\def \fxp { \simr(\bx') }
\def \gx { \bg(\bx) }
\def \gxp { \bg(\bx') }
\def \ux { \bu(\bx) }
\def \uxp { \bu(\bx') }
\def \vx { \bv(\bx) }
\def \vxp { \bv(\bx') }
\def \wx { \bw(\bx) }
\def \wxp { \bw(\bx') }
\def \yx { \by(\bx) }
\def \yxp { \by(\bx') }
\def \yX { \by(\bX) }
\def \yXp { \by(\bX') }
\def \ykx { y_k(\bx) }
\def \ylxp { y_l(\bx') }
\def \cX { \bc(\bX) }
\def \cXp { \bc(\bX') }
\def \fX { \simr(\bX) }
\def \fXp { \simr(\bX') }
\def \gX { \bg(\bX) }
\def \gXp { \bg(\bX') }
\def \uX { \bu(\bX) }
\def \uXp { \bu(\bX') }
\def \vX { \bv(\bX) }
\def \vXp { \bv(\bX') }
\def \wX { \bw(\bX) }
\def \wXp { \bw(\bX') }


% Dispersion and DDR
\def \disp { d }
\def \dr { \rho }
\def \ddr { h }
\def \zSM { z_{SM} }
\def \zWD { z_{WD} }
\def \zWS { z_{WS} }
\def \dispin { \disp( \cin ) }

% Definitions for ease-of-notation-change if need be.
\def \simulator { f }
\def \mean { \mu }
\def \cl { \theta }
\def \meanvec { \bm{ \mu } }
\def \varmat { \bm{ \nu } }
\def \dist { \pi }

% sequences
\newcommand{\seq}[2]{#1,\dots,#2}
\newcommand{\seqsub}[3]{\seq{#1_{#2}}{#1_{#3}}}
\newcommand{\seqsup}[3]{\seq{#1^{#2}}{#1^{#3}}}
\newcommand{\seqsupb}[3]{\seqsup{#1}{(#2)}{(#3)}}
\newcommand{\funseq}[4]{\seq{#1_{#3}(#2)}{#1_{#4}(#2)}}
\newcommand{\fundes}[4]{\seq{#1(#2^{(#3)})}{#1(#2^{(#4)})}}
\newcommand{\fundesT}[4]{\seq{#1(#2_{#3})^T}{#1(#2_{#4})^T}}
\newcommand{\fundesiT}[5]{\seq{#1(#2^{#3(#4)})^T}{#1(#2^{#3(#5)})^T}}

% nomenclature
\newcommand{\nom}[2]{\nomenclature{$ #1 $}{#2}}

% Bayes linear calculations
\def \bOi { \bO^{-1}  } % Omega inverse.
\def \bDi { \bDe^{-1} }
\def \eb { \ed{\bF}{\bb} } % adjusted expectation for beta.
\def \ebt { \ed{\bF}{\bb^T} } % adjusted expectation for beta.
\def \vb { \vard{\bF}{\bb} } % adjusted variance for beta. 
\def \ewX { \e{\wX} } % expectation of w(X)
\def \vwX { \var{\wX} } % variance of w(X)
\def \WDW { \bW \, \bDe \, \bW^T }
\def \WOW { \bW^T \, \bOi \, \bW }
\def \WO { \bW^T \, \bOi }
\def \DG { \bDi \bGa }
\def \bbgls { \hat{\bb}_{GLS} }
\def \GCG { \bG^T \, \bC^{-1} \, \bG }
\def \GC { \bG^T \, \bC^{-1} }
\def \IxG  { ( \identity_q \otimes \bG ) }
\def \IxGt { ( \identity_q \otimes \bG^T ) }
\def \SxC { ( \Sig \otimes \bC ) }
\def \wix { \bw_i(\bX) }
\def \wjx { \bw_j(\bX) }

% New line
\newcommand{\NL}{ \nonumber \\ &&  \,\,\,\,\,\, } 
\newcommand{\NLeq}{ \nonumber \\  &=&} 












































